Hierarchical Inference of the Lensing Convergence from Photometric Catalogs with Bayesian Graph Neural Networks

We present a Bayesian graph neural network (BGNN) that can estimate the weak lensing convergence ($\kappa$) from photometric measurements of galaxies along a given line of sight. The method is of particular interest in strong gravitational time delay cosmography (TDC), where characterizing the "external convergence" ($\kappa_{\rm ext}$) from the lens environment and line of sight is necessary for precise inference of the Hubble constant ($H_0$). Starting from a large-scale simulation with a $\kappa$ resolution of $\sim$1$'$, we introduce fluctuations on galaxy-galaxy lensing scales of $\sim$1$''$ and extract random sightlines to train our BGNN. We then evaluate the model on test sets with varying degrees of overlap with the training distribution. For each test set of 1,000 sightlines, the BGNN infers the individual $\kappa$ posteriors, which we combine in a hierarchical Bayesian model to yield constraints on the hyperparameters governing the population. For a test field well sampled by the training set, the BGNN recovers the population mean of $\kappa$ precisely and without bias, resulting in a contribution to the $H_0$ error budget well under 1\%. In the tails of the training set with sparse samples, the BGNN, which can ingest all available information about each sightline, extracts more $\kappa$ signal compared to a simplified version of the traditional method based on matching galaxy number counts, which is limited by sample variance. Our hierarchical inference pipeline using BGNNs promises to improve the $\kappa_{\rm ext}$ characterization for precision TDC. The implementation of our pipeline is available as a public Python package, Node to Joy.

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar
#
# Alex Drlica-Wagner: https://github.com/LSSTDESC/start_paper/issues/new?body=@kadrlica

# Primary file names - avoid cookiecutter variables, to enable `make
# upgrade` to cleanly over-write this Makefile...
main ?= main
#default=$(shell cat .metadata.json | grep 'default_format' | cut -d'"' -f4)
outname ?= $(notdir $(shell pwd))

#ifeq ($(default), {{ cookiecutter.default_format }})
style ?= lsstdescnote
#else
# style=${default}
#endif

# 'note' shall be an alias for 'lsstdescnote'
ifeq ($(style),note)
style = lsstdescnote
endif
# mkauthlist doesn't recognize lsstdescnote as a style, so tell it to do something generic
ifeq ($(style),lsstdescnote)
mastyle = tex
else
mastyle = $(style)
endif

DESCTEX := desc-tex
DESCTEXORIGIN := https://github.com/LSSTDESC/desc-tex.git
LSSTTEX := lsst-texmf
LSSTTEXORIGIN := https://github.com/lsst/lsst-texmf.git

localpip ?= F
PIPOPTS = --upgrade-strategy only-if-needed
ifeq ($(localpip),T)
MKAUTHBIN := bin/mkauthlist
MKAUTH := PYTHONPATH=$$(ls -d lib/python*/site-packages 2>/dev/null | head -n1):$$PYTHONPATH $(MKAUTHBIN)
PIPOPTS += --install-option="--prefix=$(PWD)"
GETMKAUTH := [ -e $(MKAUTHBIN) ] || pip install $(PIPOPTS) mkauthlist
else
MKAUTHBIN :=
MKAUTH := mkauthlist 
GETMKAUTH := pip list 2>/dev/null | grep -q mkauthlist || pip install $(PIPOPTS) mkauthlist
endif

# LATEX environment variables
export TEXINPUTS:=./$(DESCTEX)/styles/:./tables/:
export BSTINPUTS:=./$(DESCTEX)/bst/:
export BIBINPUTS:=./$(DESCTEX)/bib/:./$(LSSTTEX)/texmf/bibtex/bib/:

# LaTeX journal class switcher flags
# apj=\def\flag{apj}
# apjl=\def
# mnras=\def\flag{mnras}

# Submission flags (these need some thought)
# arxiv=\def\flag{emulateapj}
# submit=${aastex}
# draft=\def\linenums{\linenumbers}

# Files to copy when making tarball
tardir := tmp
figdir ?= ./figures
figures ?= $(figdir)/*.{png,jpg,pdf}
tabdir ?= ./tables
tables ?= $(tabdir)/*.tex
styles ?= ./$(DESCTEX)/styles/*.{sty,cls}
bibs ?= ./$(DESCTEX)/bib/*.bst
source = $(main).{tex,bbl,bib} $(DESCTEX)/bib/lsstdesc.bib $(DESCTEX)/ack/*.tex authors.tex contributions.tex $(LSSTTEX)/texmf/bibtex/bib/lsst.bib $(LSSTTEX)/texmf/bibtex/bib/lsst-dm.bib

tarfiles = $(figures) $(tables) $(styles) $(bibs) $(source)

# prefix for difference files
DIFPRE ?= diff_
# git repo branch to compare changes against
BASEBRANCH ?= master
# git repo branch we are compiling
THISBRANCH := $(shell git branch --no-color 2> /dev/null | sed -e '/^[^*]/d' -e 's/* \(.*\)/ \1/' | tr -d ' ')
# temp file for the version to compare against
DRAFT = $(main).$(BASEBRANCH)
# base for difference files to generate
DIFF = $(DIFPRE)$(THISBRANCH)--$(BASEBRANCH)


maketargets := all authlist clean copy diff help $(main) update tar templates tidy touch
.PHONY: $(maketargets)

styleopts := aastex61 apj apjl emulateapj lsstdescnote mnras note prd prl tex 
help:
	@echo "Usage: make [style=lsstdescnote] [localpip=F] <target(s)>\n Possible targets: $(maketargets) <style> $(DESCTEX) $(LSSTTEX)\n  all: equivalent to 'make $(main) copy'\n  authlist: use mkauthlist to generate latex author/affiliation listing\n  clean: remove latex temporary files AND compiled outputs\n  copy: copy $(main).pdf to $(outname).pdf\n  diff: if we're in a git repo, use latexdiff to compare the current $(main).tex vs the $(BASEBRANCH) branch, and attempt to compile to $(DIFF).pdf\n  help: what you're looking at\n  $(main): compile $(main).tex\n  update: update desc-tex, mkauthlist, and templates repo\n  tar: tar up latex source files to $(outname).tar.gz\n  templates: download latest templates to templates/\n  tidy: delete latex temporary files\n  touch: touch $(main).tex to force a recompile\n  <style>: equivalent to 'make style=<style> $(main) copy tar' (see style option)\n  $(DESCTEX): download $(DESCTEX), which provides the DESC header logo and latex helper files (done automatically on first latex compilation)\n  $(LSSTTEX): download $(LSSTTEX), providing (among other things) LSST project bib files (not done automatically)\n Options for style: $(styleopts) (Anything else results in generic latex)\n Options for localpip: T or F. Set to T to install mkauthlist in this directory rather than systemwide"


# Interpret `make` with no target as `make tex` (a latex Note).
# At present, if the default_format is anything other than
# [apj|apjl|mnras|prd|prl|emulateapj], a latex Note is made.
# In future, we could think of using `make` to eg run the ipynb
# notebook and make PDF from the output, but this has not been
# implemented yet.
$(main): export flag = \def\flag{${style}}
envflag = \\def\\flag{${style}}
all: $(main) copy

copy:
	cp ${main}.pdf ${outname}.pdf

touch:
	touch ${main}.tex

# if we are in a git repo, add as a submodule; otherwise clone
$(DESCTEX):
	if [ -d .git ]; then git submodule add $(DESCTEXORIGIN); else git clone $(DESCTEXORIGIN); fi
$(LSSTTEX):
	if [ -d .git ]; then git submodule add $(LSSTTEXORIGIN); else git clone $(LSSTTEXORIGIN); fi

#http://journals.aas.org/authors/aastex/linux.html
#change the compiler call to allow a "." file
# {% raw %}
$(main) : $(DESCTEX) authlist
	STYLEFLAG=$(envflag) latexmk $(main)
#	latexmk -g -pdf  \
	-pdflatex='openout_any=a pdflatex %O -interaction=nonstopmode "${flag}\input{%S}"'  \
	${main}
# {% endraw %}

diff: $(DIFF).pdf
$(DIFF).pdf: $(DIFF).tex
	STYLEFLAG=$(envflag) latexmk $<
$(DIFF).tex: $(DRAFT).tex $(main).tex
	latexdiff --exclude-textcmd="multicolumn" $^ > $@
# this ensures that the version to latexdiff against is always updated
.PHONY: $(DRAFT).tex
$(DRAFT).tex:
	if git show $(BASEBRANCH):$(main).tex > $@; then true; else echo "\n\n'make diff' is intended to be used inside a git repository\n"; false; fi



tar : $(main)
	mkdir -p ${tardir}
	cp ${tarfiles} ${tardir} | true
	cp ${outname}.pdf ${tardir}/${outname}.pdf
	cd ${tardir} && tar -czf ../${outname}.tar.gz . && cd ..
	rm -rf ${tardir}

authlist: authors.tex
authors.tex : authors.csv
	$(GETMKAUTH)
	$(MKAUTH) -j ${mastyle} -f -c "LSST Dark Energy Science Collaboration" \
		--cntrb contributions.tex authors.csv authors.tex
#	pip install --upgrade mkauthlist


# http://stackoverflow.com/q/8028314/
.PHONY: $(styleopts)
$(styleopts): export style = $(@)
$(styleopts): export flag = \def\flag{$(@)}
$(styleopts):
	$(MAKE) -e $(main)
	$(MAKE) -e copy
	$(MAKE) -e tar
# NB. the 'tex' target doesn't actually do anything in docswitch - make
# with no target compiles PDF out of main.tex using lsstdescnote.cls
# (which is to say, by default we assume you are writing an LSST
# DESC Note in latex format).

tidy:
	rm -f *.log *.aux *.out *.dvi *.synctex.gz *.fdb_latexmk *.fls
	rm -f *.bbl *.blg *Notes.bib ${main}.pdf

clean: tidy
	rm -f ${outname}.pdf ${outname}.tar.gz

# Update the tex styles etc:

baseurl=https://raw.githubusercontent.com/LSSTDESC/start_paper/deploy

# UPDATES=\
# texmf/bib/apj.bst \
# texmf/bib/mnras.bst \
# texmf/styles/aas_macros.sty \
# texmf/styles/aastex.cls \
# texmf/styles/aastex61.cls \
# texmf/styles/aps_macros.sty \
# texmf/styles/docswitch.sty \
# texmf/styles/emulateapj.cls \
# texmf/styles/mnras.cls \
# texmf/styles/lsstdescnote.cls \
# texmf/styles/lsstdesc_macros.sty \
# texmf/logos/desc-logo-small.png \
# texmf/logos/desc-logo.png \
# texmf/logos/header.png \
# lsstdesc.bib \
# .travis.yml \
# figures/example.png

# .PHONY: $(UPDATES)
# $(UPDATES):
# 	curl -s -S -o $(@) ${baseurl}/$(@)
# 	@echo " "

update: templates
	@echo Updating desc-tex
	cd $(DESCTEX) && git pull
	@echo
	@echo Updating mkauthlist
	pip install --upgrade $(PIPOPTS) mkauthlist
#@echo "\nOver-writing LaTeX style files with the latest versions: \n"
#@mkdir -p .logos figures texmf/styles texmf/bib
#$(MAKE) $(UPDATES)

# Get fresh copies of the templates etc, for reference:
# It is a bad idea to make these phony targets

TEMPLATES:=\
authors.csv \
main.ipynb \
main.md \
main.rst \
main.tex \
main.bib \
Makefile
#.metadata.json \
#.travis.yml 
#figures/example.png
# #acknowledgments.tex \

ALLTEMPLATES := $(TEMPLATES) header.png

# .PHONY: $(TEMPLATES)
# $(TEMPLATES):
# 	curl -s -S -o templates/$(@) ${baseurl}/$(@)
# 	@echo " "

gettemplates := $(foreach t,$(TEMPLATES),curl -s -S -o templates/$(t) ${baseurl}/$(t); )

# NB: fetching header.png will fail as long as desc-tex is private
templates:
	@echo "\nDownloading the latest versions of the template files, for reference: \n"
	@mkdir -p templates
	$(gettemplates)
	curl -f -s -S -o templates/header.png https://raw.githubusercontent.com/LSSTDESC/desc-tex/master/logos/header.png || true
	@echo
	@echo templates/ listing:
	@ls -a templates/*
	@for f in $(ALLTEMPLATES); do diff -q $$f templates/$$f; true; done
#$(MAKE) $(TEMPLATES)
#	$(MAKE) new

# Get a template copy of the latest Makefile, for reference:
# new:
# 	@echo "\nDownloading the latest version of the Makefile, for reference: \n"
# 	@mkdir -p templates
# 	curl -s -S -o templates/Makefile ${baseurl}/Makefile
# 	@echo " "

# Over-write this Makefile with the latest version:
# Why would we include this when a safe option already exists?
# upgrade:
# 	@echo "\nDownloading the latest version of the Makefile: \n"
# 	curl -s -S -o Makefile ${baseurl}/Makefile
# 	@echo "\nUpgrading version of mkauthlist: \n"
# 	pip install mkauthlist --upgrade --no-deps
# 	@echo "\nNow get the latest styles and templates with\n\n    make update\n    make templates\n"


==> authors.tex <==



==> desc-tex/ack/key.tex <==
The DESC acknowledges ongoing support from the Institut National de Physique Nucl\'eaire et de Physique des Particules in France; the Science \& Technology Facilities Council in the United Kingdom; and the Department of Energy, the National Science Foundation, and the LSST Corporation in the United States.  DESC uses resources of the IN2P3 Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la Recherche Scientifique; the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported by the Office of Science of the U.S.\ Department of Energy under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BIS National E-infrastructure capital grants; and the UK particle physics grid, supported by the GridPP Collaboration.  This work was performed in part under DOE Contract DE-AC02-76SF00515.


==> desc-tex/ack/standard_short.tex <==
DESC acknowledges ongoing support from the IN2P3 (France), the STFC (United Kingdom), and the DOE, NSF, and LSST Corporation (United States).  DESC uses resources of the IN2P3 Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la Recherche Scientifique; the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BIS National E-infrastructure capital grants; and the UK particle physics grid, supported by the GridPP Collaboration.  This work was performed in part under DOE Contract DE-AC02-76SF00515.


==> latexmkrc <==
# Choose which style to pass to docswitch
# NB: Default value here is always used by Overleaf
$theflag = $ENV{'STYLEFLAG'} || '\def\flag{lsstdescnote}';

# Set environment variables to search for tex inputs
# http://tex.stackexchange.com/a/50847/121099
$ENV{'TEXINPUTS'}='./desc-tex/:./tables/:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./desc-tex/bib/:' . $ENV{'BSTINPUTS'};

# Set control tools
$go_mode = 1;
$pdf_mode = 1;
# You can change the \flag value here...
$pdflatex = 'openout_any=a pdflatex %O -interaction=nonstopmode "' . $theflag . '\input{%S}"'


==> sections/intro.tex <==
% usefulness of strong lensing (focus on time delays cosmography?), MSD. it's bad -- will get to it later.
Strong lensing time delay systems provide a direct measurement of the physical scales along a particular line of sight (LOS). They represent a unique cosmographic probe that yields measurements of the Hubble constant ($H_0$) fully independently of local distance ladder methods and early-universe probes like the cosmic microwave background (CMB). With high signal-to-noise ratio (SNR) and high-resolution imaging of the lensed source, a detailed mass model of the deflector galaxy can be obtained. The integrated structure along the LOS, however, introduces weak lensing perturbations that affect the time delays while keeping imaging observables the same under linear transformations of the lens equation -- the so-called mass-sheet degeneracy (MSD).

% MSD 
As shown in \cite{falco1985model}, remapping the reference mass distribution $\kappa$, for any scalar $\lambda$, as
\begin{equation}
    \label{eq:msd}
    \kappa_{\lambda}(\theta) = \lambda \kappa(\theta) + (1 - \lambda)
\end{equation}
 while isotropically scaling the source plane as $\beta \rightarrow \lambda \beta$ results in the same dimensionless observables (image pixel values) but different time delays. The infinite family of solutions to the lens equation results in a range of inferred properties of the deflector and the source. The additional mass term in \ref{eq:msd} is either internal to the main deflector and affects its kinematics or due to the external LOS structure. It is common practice to express the external portion as an equivalent additional mass sheet at the redshift of the main deflector with uniform surface mass density called external convergence, denoted $\kappa_{ext}$ \citep{schneider1997cosmological, keeton1997shear}.

The parameter $\kappa_{ext}$ 
%What the previous work found: 1. photometric catalogs have enough info! 2. uncertainty increases with increasing kappa, raises concern because lenses are massive and tend to be in dense environments

%Problems with previous work 
%CDE; loss function

%I see your project as solving the major problems with that approach, which was correct in principle but was fatally held back by our inability to handle the mass model of the light cone towards each lens. The DNN should be able to learn this model internally in a way our simple Pangloss model just wasn’t. In particular, we won’t have to a) assume an overly simple model for the distribution of dark matter in galaxies and clusters, or b) correct for the mass that is not in galaxy or cluster halos.

%Goal: P(kappa) at a specific location in the sky (lens) averaged over the scale of the Einstein radius not accounting for the explicitly modeled structure (lens model)

%Approach:Estimator from the luminous tracers of the underlying matter field with a prior on the expected relation and scatter P(kappa | luminous structure). Prior is based on a dark matter only simulation (Millenium simulation) Dedicated imaging and spectroscopical campaigns are made to gather as much as possible information about the specific line of sight.

%Insufficiencies (sorry if this is a bit a rant, I just want to make sure I list all the things that I personally have my doubts and that I want to see improved):
%1. double counting of mass that is explicitly modeled in the analysis not fully self consistent (there are checks being made that this effect is small, but still)
%2. analysis relies on semi-analytic galaxy-halo models that do not necessarily reproduce the observed mass/luminosity function (-> universe machine/Buzzard) (this might not be a too large problem as in the current summary statistics only relative quantities in respect to a control field are used, but still)
%3. ad-hoc summary statistics (weighted galaxy counts within certain annuli) rather than robust checks for an informative and unbiased summary statistics (there has not been made a single! validation of wether the current summary statistics leads to unbiased results when analyzing a population of lenses)
%4. I formulated in the J1206 work last year the current analysis within the framework of Approximate Bayesian Computing (ABC). Before that any proper Bayesian interpretation of the selected line of sights was lacking and I realized that their treatment of selecting specific line of sights was not a rigorous Bayesian approach.
%5. The lens is often a massive elliptical galaxy and it’s physical environment may be part of a larger group. There are dedicated spectroscopic campaigns to get exquisites redshifts/relative velocity do quantify physically bound systems. The interpretation of the relative velocities and numbers of galaxies is severely limited. Only in the very high S/N regime with dozens of galaxies in a well structured velocity and position space, very reliable conclusions can be drawn. There is no back up on simulations in the interpretation of the spectroscopic data. The problem here is as well as there is no control field with comparable spectroscopic coverage and depth.
%6. Lack of proper stellar-halo mass connection with incorporation of stellar velocity dispersion to assess biases in the mass estimates of the lenses (highly relevant also for the lensing substructure work). But this requires the stellar-halo mass model to self-consistently incorporate stellar velocity dispersion as well as this is a more direct observable of the potential depth of the halo.

%Not done (yet):7. LOS correction to the lens plane itself (I pointed that out two years ago but has not been tackled)
%8. Non-linear effect of the LOS between lens and source plane (it’s just a correction factor in the lensing kernel due to the foreground bending of the light ray where the Born approximation fails and needs to be replaced with two different Born approximations)
%9. Weak lensing has been proposed to be added to the observables that can help characterize the LOS but it has not been implemented self-consistently.

%Basically, we can write a paper laying out a proper way of performing an unbiased estimator for P(kappa) based on simulations and validated by them. We may or may not also incorporate the current analysis to point out how much a potential bias is (if it’s worth) or being simply the leading group that does the re-analysis of the current lensing sample with the improved approach (after writing a first method paper). At the end, a paper could be very straight forward (at least in wording):
%1. We use/calibrate the Buzzard simulations on a specific data set 2. We train a neural network on predicting P(kappa) at different mock observed LOS of the simulation 3. We validate the unbiased recovery of the predicted P(kappa) 4. We apply the technique on one or two lenses (why not the current one in the DES footprint?)
